milliEgo: Single-chip mmWave Radar Aided Egomotion Estimation via Deep Sensor Fusion

Robust and accurate trajectory estimation of mobile agents such as people and robots is a key requirement for providing spatial awareness for emerging capabilities such as augmented reality or autonomous interaction. Although currently dominated by optical techniques e.g., visual-inertial odometry, these suffer from challenges with scene illumination or featureless surfaces. As an alternative, we propose milliEgo, a novel deep-learning approach to robust egomotion estimation which exploits the capabilities of low-cost mmWave radar. Although mmWave radar has a fundamental advantage over monocular cameras of being metric i.e., providing absolute scale or depth, current single chip solutions have limited and sparse imaging resolution, making existing point-cloud registration techniques brittle. We propose a new architecture that is optimized for solving this challenging pose transformation problem. Secondly, to robustly fuse mmWave pose estimates with additional sensors, e.g. inertial or visual sensors we introduce a mixed attention approach to deep fusion. Through extensive experiments, we demonstrate our proposed system is able to achieve 1.3% 3D error drift and generalizes well to unseen environments. We also show that the neural architecture can be made highly efficient and suitable for real-time embedded applications.

==> sections/att_fuse.tex <==
%!TEX root = ../main.tex
\section{Multi-modal Odometry Fusion} % (fold)
\label{sec:multi_modal_odometry}

So far we have discussed how \monet estimates the ego-motion with a low-cost mmWave radar. In the real world, mobile agents are often outfitted with multiple sensors. For instance, a smartphone is equipped with a combination of GPS, IMUs, monocular or stereo video cameras and even mmWave radars \cite{pixel4} that collectively achieve task goals. Under this context, we now introduce how to effectively combine mmWave radar with other available sensors to obtain a more accurate odometry.  
The key observation made in this section is that, \emph{owning to the dynamic observation quality, treating different odometry sensors evenly in a deep network results in sub-optimal estimation and lacks robustness against environment uncertainty}. In what follows we start by illustrating the fusion challenge and then describe our proposed attention mechanism to combat it.

\subsection{Challenge of Fusing Deep Features} % (fold)
\label{sub:challenge_of_direct_fusion}

% lack of physical intervention f
A robust odometry obtained by fusion is based on the complementary interactions amongst different sensors, whose roles are adaptively altered or weighted in response to observation uncertainties or self/environmental dynamics. For example, inertial sensors should dominate odometry estimation against RGB cameras under strong lightning changes, lack of textures and high-speed motions.
Classical sensor fusion algorithms realized such adaption by incorporating physical models into the algorithm design, e.g., Bayesian filtering or fixed-lag smoothers. However, adaptive fusion strategies are still under-explored when it comes to deep feature space, such as the deep mmWave odometry \monet. Notably, this deep future space is not only driven by our \monet but also influenced by other sensors. To avoid hand-crafted feature engineering, prevalent odometry systems, e.g., Visual Odometry (VO) or Inertial Odometry (IO), are increasingly adopting deep neural networks for end-to-end estimation, leaving fusion operations all inside the deep feature space. The challenge a multi-modal odometry faced here is boiled down to that one can hardly incorporate an adaptation mechanism, which is often inspired from ambient physics, into a black box model due to DNN's multilayer nonlinear structure. 

\begin{figure}[!t]
	\centering
	\includegraphics[width=\columnwidth]{figures/attention_mech.pdf} 
\caption{Architectural Comparison between single-stage attention mechanism and our proposed mixed (two-stage) attention mechanism.}
\label{fig:attention_mech}
\end{figure}

\subsection{\atfuse: Mixed Attention for Fusion} % (fold)
\label{sub:mixed_attention_for_fusion}

To endow a multimodal deep odometry that adapts to environmental uncertainties, we propose \textbf{\atfuse}, moving from automatic feature extraction to autonomous network behavior change. Critical to \atfuse is its mixed attention mechanism, which realized model adaptation through mixed attention module. As shown in Fig.~\ref{}, \atfuse a self-attention layer and a cross-modal attention layer. These two attention layers are essentially two feature masks that respectively discover intra-level feature correlation and inter-level feature correlation. Our key observation underpinning the use of mixed attention is: \emph{complementary sensor interactions are best realized in the deep feature space by different attention operations in tandem}. Concretely, the proposed mixed attention module comprises a \emph{self-attention} module handling the intra-level interaction within individual sensors, and a \emph{cross-modal attention} module coping with the inter-level interaction across sensor modalities.

\subsection{Intra-sensor Self-Attention} % (fold)
\label{sub:self_fusion_for_intra_feature_correlation}

\noindent \textbf{Motivation}.
A promising direction to enable the aforementioned odometry model to adapt is letting those deep features automatically generate masks for and use masks to filter themselves. This idea conceptually falls into the technique of `self-attention', which was initially designed for machine translation and image transformer to address the long dependency issue \cite{vaswani2017attention,dou2019dynamic,parmar2018image}. Inspired by these early successes, we consider using the self-attention mechanism to realize odometry self-regulation. Particular, without resorting to the complex query-key-value pipeline in \cite{vaswani2017attention}, we adopt a space/spacetime non-local framework akin to \cite{wang2018non}) which is proven to adaptively re-weighs feature importance.  

\noindent \textbf{Self-attention}.
For the ease of illustration, we start by attending the features of our mmWave odometry. Given an extracted feature vector $\mathbf{z}_M$ produced by \monet (i.e., the features extracted by the CNN extractor introduced in \sect{\ref{sub:network_architecture}}), a self-attention module first computes the similarity between two embedding spaces and uses the similarity to generate an attention map:
\begin{equation}
     \mathbf{a}_M = \sigma[(\mathbf{W}_M^\varrho \mathbf{z}_M)^{T} \mathbf{W}_M^\varphi \mathbf{z}_M]
\label{eq:self-att}
\end{equation}     
\noindent where $\mathbf{W}_M^\varrho$ and $\mathbf{W}_M^\varphi$ are learnable weight matrices that project the original features to embededing spaces $\varrho(\mathbf{z}_M)$ and $\varphi(\mathbf{z}_M)$ respectivly. $\sigma$ represents a non-linear activation function, e.g., softmax or sigmoid. After applying the generated focus mask, the attended features $\mathbf{\tilde{z}}_M$ is given:
\begin{equation}
     \mathbf{\tilde{z}}_M = \mathbf{a}_M \odot \mathbf{z}_M
\end{equation}  
\noindent where $\odot$ denotes element-wise multiplication. From the perspective of filtering, self-attention enforces the model to focus on stable and geometry meaningful features yet ignore distracting components, so as to regulate the estimation model in response to complex environment uncertainty. In this way, we can similarly generate the self-regulated deep odometry features for inertial sensors ($\mathbf{\tilde{z}}_I$), RGB cameras ($\mathbf{\tilde{z}}_V$) or depth cameras ($\mathbf{\tilde{z}}_D$) depending on their availability.
As introduced in \cite{wang2018non,vaswani2017attention}, through the similarity comparison between two embeddings, self-attention is able to prominently capture the long-range dependencies and global correlations of the features. This feature is of paramount importance for odometry estimation, where widely separated spatial regions should jointly considered. In contrary, convolution layers (broadly are filters as well) only operate on a limit-size receptive field, incommensurate to our goal of re-weighting features globally. It justifies the non-redundant role of self-attention. 
% Compared to other sensors, we found that the self-attention layer is of paramount importance to \monet, owning to the significant noise level in mmWave data. By using the self-attention mask, the odometry network model can further improve the stability by focusing on the informative components as illustrated in Fig.~\ref{mmwave_self_attention}. 

\todo{add a attention map figure}

\subsection{Inter-sensor Cross-Attention} % (fold)
\label{sub:cross_modal_fusion}

\noindent \textbf{Motivation}.
Self-attention layer re-weighs importance of intra-sensor descriptors in the deep feature space. We now extend this idea to inter-sensor correlations. The cross-attention serves as the second-stage re-weighting, which is inspired by the mechanism of human perception. Specially, when one of five our senses drops out, another can pick up the slack. A typical example is people who are blind can train and use their hearing to play double duty \cite{cappagli2017auditory}. Our senses regularly meet and \emph{crosstalk} in the brain to provide accurate impressions of the world \cite{bleicher2012edges,seubert2012know}. Analogously, we expect a multi-modal odometry system to adaptively shift contributive roles against different challenging scenarios. For example, the odometry branch from \monet should automatically take over the estimation when a co-located RGB camera encounters strong lighting changes (e.g., darkness or dimness).

\noindent \textbf{Cross-attention}.
To make these odometry sensors ``crosstalk'' to each other, we consider generating attention masks across sensor descriptors, where the conditioning process is akin to self-attention. To bootstrap the explanation, we start with the case combining mmWave radar with inertial sensor. Given their features $\mathbf{\tilde{z}}_M$ and $\mathbf{\tilde{z}}_I$ after self-attention, two respective cross-attention masks are derived as follows:
\begin{equation}
\begin{split}
	\mathbf{a}_{I \rightarrow M} &= \sigma[(\mathbf{W}_{I \rightarrow M}^\varrho   \mathbf{\tilde{z}}_I)^{T}\mathbf{W}_{I \rightarrow M}^\varphi   \mathbf{\tilde{z}}_I] \\
	\mathbf{a}_{M \rightarrow I} &= \sigma[(\mathbf{W}_{M \rightarrow I}^\varrho   \mathbf{\tilde{z}}_M)^{T}\mathbf{W}_{M \rightarrow I}^\varphi   \mathbf{\tilde{z}}_M]
\end{split}
\end{equation}  	
where the family of $\mathbf{W}$ are learnable weight matrices. The final multi-modal odometry descriptors can be modeled by concatenating the second-stage attended features:
\begin{equation}
	\mathbf{\bar{z}}_{MI} = [\mathbf{a}_{M \rightarrow I} \odot \mathbf{\tilde{z}}_I; \mathbf{a}_{I \rightarrow M} \odot \mathbf{\tilde{z}}_M]
\end{equation}
When more than two odometry sensors are available, e.g., mmWave radars ($\mathbf{\tilde{z}}_M$), inertial sensors ($\mathbf{\tilde{z}}_I$) and RGB cameras ($\mathbf{\tilde{z}}_V$), we can randomly leave one out first and concatenate the rest of them and then generate an attention mask conditioned on it. In an example generating mmWave attention mask from RGB and inertial sensors, this can be described as:
\begin{equation}
  	\mathbf{a}_{VI \rightarrow M} = \sigma[(\mathbf{W}_{VI \rightarrow M}^\varrho   \mathbf{\tilde{z}}_{VI})^T\mathbf{W}_{VI \rightarrow M}^\varphi   \mathbf{\tilde{z}}_{VI}]
\label{eq:cross-att}
\end{equation}  
where $\mathbf{\tilde{z}}_{VI} = [\mathbf{\tilde{z}}_{V}; \mathbf{\tilde{z}}_{I}]$, which are the concatenated features from two sensors after self-attention. The final attended features are:
\begin{equation}
	\mathbf{\bar{z}}_{MIV} = [\mathbf{a}_{MV \rightarrow I} \odot \mathbf{\tilde{z}}_I; \mathbf{a}_{VI \rightarrow M} \odot \mathbf{\tilde{z}}_M; \mathbf{a}_{MI \rightarrow V} \odot \mathbf{\tilde{z}}_V]
\end{equation}
This finishes the mixed attention. The final attended features are fed into the follow-up RNN module and FC pose regressors, as introduced in \sect{\ref{sub:network_architecture}}. 

\subsection{Discussion of Mixed Attention} % (fold)
\label{sub:discussion_of_mixed_attention}

\atfuse is essentially a two-stage attention framework that operates in tandem. A natural thought, however, is why not concatenating the extracted features from CNN modules into a ``big'' merged vector, and just performing the self-attention on it. In this way, the role of the cross-attention is expected to be surrogated into the ``big'' mask generated by self attention, leaving to a single-stage framework. We now justify this two-stage attention from the perspectives of both effectiveness and efficiency. 

\noindent \textbf{Effectiveness}.
Recall the end goal of attention is to realize the adaption ability through complementary sensor interactions of a multi-modal odometry system. Although \sect{\ref{sec:evaluation}} will further confirm such effectiveness from quantitative results, a more intuitive way to examine is by visualizing some generated masks and validate their behavior changes in different scenarios. As we can see in Fig.~\ref{}, the masks of different sensors generated by a single-stage attention does not indicate cross-modal complementariness and change \emph{synchronously} over time. By inspecting the data, we found that, the concurrent weight increasing for all sensors is probably due to one of them got activated in response (e.g., turning for inertial sensors). However, as the network treats all elements in the `big' feature vector evenly without considering their provenance, synchronous weight change happens and leaves complementary behavior hard to achieve.
In contrast, the focus maps generated by our two-stage attention strategy give rise more complementary behaviors. In particular, we can clearly see that in a case with abrupt lighting change, the mask of RGB cameras automatically tunes down its contribution while the weights of other two sensors get enlarged. \todo{give a figure to illustrate}.
We hypothesize that by disentangling attention modeling, the individuality of sensors can be best preserved as each of them has a separate mask for its features. Such individuality arguably lays the basis for allowing the complementary behaviors. Note that self-attention also plays an important role in our two-stage strategy. Indeed, self-attention facilitates the follow-up cross-attention because intuitively, the filtered feature information is more reliable to be conditioned on. We will come to this point and discuss its necessity more in \sect{\ref{sec:eval}}.

\noindent \textbf{Complexity}.
We further argue that our two-stage attention does not incur further computation overheads. Take the MIV (mmWave-Inertial-Visual) odometry as example, we denote the lengths of their extracted feature vectors as $N_M$, $N_I$ and $N_V$. Inspecting Eq.~(\ref{eq:self-att}, \ref{eq:cross-att}), the total weight matrix size is $2\times(N_M+N_I+N_V)^2$ for single-stage strategy, which is same as the space complexity of our mixed attention module:
\begin{equation*}
 	\underbrace{2\times(N_M^2 + N_I^2 + N_V^2)}_\text{1. self-attention} + \underbrace{4 \times (N_MN_I + N_VN_I + N_MN_V)}_\text{2. cross-attention}
 \end{equation*} 
In fact, it has been found that by breaking learning a fat weight matrix into several smaller matrices lined up, more efficient learning and less network over-fitting can be also obtained \cite{srivastava2015training}. 

==> sections/deepmo.tex <==
%!TEX root = ../main.tex
\section{Deep Odometry Model} % (fold)
\label{sec:deep_mmwave_odometry}

As shown in Fig.~\ref{fig:milliEgo_overview}, our proposed DNN odometry model has multiple odometry subnets branching from different sensors. Although the odometry models with other sensors, such as IMU and cameras are established, the effectiveness of using mmwave data for odometry estimation remains widely unknown. As such, we will first elaborate the modeling challenge raised by the low-cost mmWave radar and then introduce our solution to address it.

In this section, we explore the feasibility of using a low-cost mmWave radar for ego-motion estimation, answering the question: \emph{is it possible to build up an usable odometry from the very sparse and noisy mmWave point clouds?}. Not only can this understanding allow the design of a standalone mmWave odometry, but provide insights for more effective sensor fusion in \sect{\ref{sec:multi_modal_odometry}}. In what follows, we start by introducing the technical challenges brought by low-quality point clouds and then describe our proposed deep learning based odometry model to address them. 

\subsection{Challenge: Chaotic Correspondences} % (fold)
\label{sub:chaotic_point_correspondences}

\begin{figure}[!t]
	\centering
	\begin{subfigure}[b]{0.24\textwidth}\centering
		\includegraphics[width=\columnwidth]{figures/pcl/lidar_before.pdf} 
		\caption{Before Registration}
		\label{fig:lidar_before}
	\end{subfigure}%
	\begin{subfigure}[b]{0.24\textwidth}\centering
		\includegraphics[width=\columnwidth]{figures/pcl/lidar_after.pdf} 
		\caption{After Registration}
		\label{fig:lidar_after}
	\end{subfigure}%
\caption{Point registration on lidar point cloud.}
\label{fig:lidar_icp}
\end{figure}

\begin{figure}[!t]
	\centering
	\begin{subfigure}[b]{0.24\textwidth}\centering
		\includegraphics[width=\columnwidth]{figures/pcl/mmwave_before.pdf} 
		\caption{Before Registration}
		\label{fig:_before}
	\end{subfigure}%
	\begin{subfigure}[b]{0.24\textwidth}\centering
		\includegraphics[width=\columnwidth]{figures/pcl/mmwave_after.pdf} 
		\caption{After Registration}
		\label{fig:lidar_after}
	\end{subfigure}%
\caption{Point registration on mmwave point cloud.}
\label{fig:lidar_icp}
\end{figure}

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.75\columnwidth]{figures/pcl/err_compare.pdf} 
	\caption{Comparing the ICP optimization error of consecutive frames.}
\label{fig:icp_error_logs}
\end{figure}

\subsubsection{Why does the challenge arise?} % (fold)
\label{ssub:why_is_the_challenge_}

As described in Sec.~\ref{sub:point_set_registration}, the point set registration between consecutive point clouds underpins odometry estimation. Critical to most registration techniques is the determination of correspondence between spatially localized 3D points within each cloud. Such registration problem is hard to solve when facing issues of noise, missing or spurious data \cite{gold1998new}, which are unfortunately the characteristics of the point cloud generated by a single-chip mmWave radar. Unlike the dense and clean data generated by lidars, the mmWave point cloud in indoor environment has two limitations: (1) multi-path noise and (2) sparsity. 

Multi-path noise is longstanding issue for almost all RF technologies, and it is exceptional for the mmWave. Concretely, the signal propagation of mmWave in indoor environments is subject to multi-path \cite{yan2016multipath} due to beam spreading and reflection from surrounding objects. As a result, reflected signals arriving at a receiver antenna are normally from two or more paths, incurring smearing and jitter. Multi-path is the primary contributor to the non-negligible proportion of pertinent noise artefacts and spurious data in the mmWave point cloud. Fig.~\ref{} shows some exemplar point clouds compromised by multi-path noise. 

On top of the strong noise, mmWave point clouds also have severe sparsity issue, owning to multiple factors resolving the low-cost single-chip design, including (i) few antennas and (ii) point aggregation mechanism. As opposite to massive MIMO radar technologies, the mmWave radar in our use only has $7$ antennas which is effective in both cost and size but fundamentally limits its spatial resolution. 
Moreover, in order to lower bandwidth burden and improve signal-to-noise ratio, commercial mmWave radars usually apply algorithms such as CFAR (Constant False Alarm Rate) \cite{ward1969handbook} in data processing and \emph{only} provide an aggregated point cloud, further reducing density. For these reasons, the resulting point clouds only contain approximately $\sim100$ reflective points per frame which is over $100\times$ sparser than a lidar. Fig.~\ref{} shows a head-to-head comparison example.


\subsubsection{What influence on odometry estimation?} % (fold)
\label{ssub:how_badly_can_the_challenge_influence_odometry_}

The above multi-path noise and sparsity issues collectively impact the registration process that makes the conventional geometry based methods fall short. The substantial noise and superiors points will make a class of voting-based registration methods ineffective \cite{huttenlocher1990recognizing}.The other established class is Iterated Closest Point algorithm (ICP) and its variants, featuring a better robustness via iteratively interleaving correspondences matching and transformation estimation. Nonetheless, ICP methods require a relative advantageous initialization, which is hard to offer now by Random sample consensus (RANSAC) \cite{hu2012robust} and other bootstrapping methods due to sparsity and lack of texture and. Additionally, its intrinsic limitation of local minima gets exacerbated as less constraints imposed in optimization \cite{bouaziz2013sparse}. Fig.~\ref{icp_fail} illustrates few failure cases of when using RANSAC-ICP algorithm for registering mmWave point clouds. As we can see, the majority of point association is false positive even after iterative optimization. These chaotic correspondences, however, lead the transformation estimation to nowhere and give disastrous odometry in the end. 

\subsection{\monet: An End-to-End Solution} % (fold)
\label{sub:monet_a_neural_network_solution}

Addressing the challenge of chaotic correspondences requires more sophisticated estimation algorithms beyond simple human heuristics. We thus propose to use deep learning based approaches which have been proved to be effective in extracting useful motion information from complicated sensor observations. Critical to this design choice is that deep learning approaches allow an end-to-end modeling fashion particularly suitable for mmWave odometry. Our key insight is: \emph{Instead of a traditional two-step registration, it is possible to directly estimate the end transformation by implicitly surrogating correspondence association in learning}. Thereby, the knock-on effect between the interleaving correspondences association and transformation estimation can be maximally mitigated. We now describe the details of our proposed \textbf{\monet} (\textbf{m}mWave \textbf{O}dometry Neural \textbf{Net}work).

\subsection{Network Inputs and Outputs} % (fold)
\label{sub:network_inputs_and_outputs}

\noindent \textbf{Inputs}.
Determining an effective input format to a neural network is non-trivial, esp. in the context of odometry estimation. Point cloud data lie in the 3D space and are unordered and irregularly sampled. Extracting the structured motion patterns from such unstructured data format is intuitively difficult, not mentioning the ambiguous orders due to severe sparsity and noise. This is probably the reason why proven networks to date designed for motion pattern extraction generally require structured inputs (e.g., \cite{ye20183d}). To this end, we encode mmWave point clouds into a 2D panoramic-view images, following the convention of \cite{li2016vehicle}: 
\begin{equation} \label{eq1}
	\begin{split}
	\alpha & = arctan2(p_y,p_x),  \quad r = \lfloor \alpha / \Delta\alpha \rfloor \\
	 \beta & = arcsin(p_z/\sqrt{p_x^2+p_y^2+p_z^2}), \quad c = \lfloor \beta / \Delta\beta \rfloor 
	\end{split}
\end{equation}
\noindent where $(p_x, p_y, p_z)$ denotes a 3D point and $(r, c)$ is the 2D map position of its projection. $\alpha$ and $\beta$ denote the azimuth and elevation angle when observing the point. $\Delta\alpha$ and $\Delta\beta$ is the average horizontal and vertical angle resolution between consecutive beam emitters respectively. After panoramic project, we further normalize their values to the range $[0, 255]$. Points closer to the sensor are assigned higher values and lower vice versa. Fig.~\ref{} illustrates an example of panoramic images. By this transformation, unstructured 3D point clouds are encoded to structured 2D images, in a similar spirits to RGB images which are tractable to many established NN feature extractors. 

\noindent \textbf{Outputs}.
Taking inputs as the stacked panoramic images ($\mathbf{x}_{k-1}$ and $\mathbf{x}_{k}$), \monet is learning a mapping function from the noisy input pairs to 6-DoF (Degree of Freedom) pose estimates $\{(\mathbf{x}_{k-1}, \mathbf{x}_{k})\} \rightarrow \{ (\mathbf{\hat{t}}_{k}, \mathbf{\hat{r}}_{k})\}$. Such output is a pair-wise relative pose while in some applications (e.g., indoor navigation etc.), the point of interest can be the global poses relative to the very initial origin so as to determined one's full movement trajectory. When global poses are needed, one can leverage a SE(3) composer \cite{wang2018end} to incrementally stitch series of relative poses into global poses.

\subsection{Network Architecture} % (fold)
\label{sub:network_architecture}

As shown in Fig.~\ref{}, the architecture of \monet is mainly composed of CNN-based feature extraction, RNN-based temporal dependency modeling and fully connected (FC) layers as pose regressor.

\noindent \textbf{CNN Feature Extractor}. Ideally the feature representation used for odometry is geometric instead of being associated with appearance or visual context. Only generic representation on geometrics can allow the learned network model generalize to unseen environments or scenarios without repetitive bespoke training. The structure of our CNN is inspired by the network for optical flow estimation \cite{dosovitskiy2015flownet}, in which the authors managed to extract effective motion flow from RGB images. We therefore also adopt the CNN structures with modification adept to our panoramic image formats. Specifically, our extractor comprises $10$ convolutional layers and each layer is followed by a Leaky version of a Rectified Linear Unit (LeakyReLU) non-linearity activation. The sizes of the receptive fields in the network gradually reduce from $7 \times 7$ to $5 \times 5$ and then $3 \times 3$ to incrementally capture smaller interesting feature. The extracted latent mmWave feature representation not only compresses the original noisy high-dim panoramic data into a compact description, but facilitates the temporal dependency modeling follows up.

\noindent \textbf{RNN Temporal Dependency Modeling}. 
On receiving the extracted features by CNN, a RNN is used to model the dynamics and relations in a sequence. Indeed, this sequential motion learning via RNNs has been recently proven to be effective for a variety of sensor modalities \cite{chen2018ionet}, ranging from inertial sensors to optical sensors, yet it is ability in modeling ego-motion from mmWave data is unveiled. 
A prominent advantage of using RNN for odometry lies in its superior ability in maintaining the memory of hidden states over long term even if the given inputs are noisy. The issue associated with RNNs, however, is that they cannot directly model high-dimensional raw sensory data such as images. But thanks to the CNN extractors, the data fed to RNN are already compressed in a low-dim space that match its capability. Specially, the RNN adopted in \monet is a two-layer Long Short-Term Memory (LSTM), each of which contains $512$ hidden units. This RNN module is on top of the CNN feature extractor layer.

\noindent \textbf{FC Pose Regressor}. 
Given the outputs of RNNs, three FC layers are introduced to regress these sequential features and predict relative transformation. These FC layers have $128$, $64$ and $6$ units respectively, with the last layer regressing all deep mmWave features into a $6$-DoF relative pose estimate:
\begin{equation}
 	\mathbf{\hat{y}}=[\mathbf{\hat{t}}, \mathbf{\hat{r}}]
\end{equation} 
\noindent where $\mathbf{\hat{y}} \in \mathbb{R}^6$. To promote model generalization ability, we also use a dropout \cite{dahl2013improving} rate of $0.25$ between FC layers to help regularization.

\subsection{Cost Function and Optimization} % (fold)
\label{sub:cost_function_and_optimization}

Training \monet is essentially optimizing the following conditional probability of the relative poses $\mathbf{Y} = (\mathbf{y}_1, \ldots, \mathbf{y}_K)$ given a sequence of panoramic images $\mathbf{X} = (\mathbf{x}_1, \ldots, \mathbf{x}_K)$:
\begin{equation}
	P(\mathbf{Y}|\mathbf{X}) = P(\mathbf{y}_1, \ldots, \mathbf{y}_K | \mathbf{x}_1, \ldots, \mathbf{x}_K)
	\label{eq:cond_prob}
\end{equation}
The modeling and probabilistic inference are implicitly performed in the DNN, by learning to find the optimal network parameters $\mathbf{\bm\theta}^{\ast}$ that maximizes Eq.~(\ref{eq:cond_prob})
\begin{equation}
	\mathbf{\bm\theta}^{\ast} = \underset{\mathbf{\bm\theta}}{\arg\max} \quad P(\mathbf{Y}|\mathbf{X}; \mathbf{\bm\theta})
\end{equation}
In the sense of Mean Squared Error (MSE), this yields our loss function which quantifies the Euclidean distance between the ground truth pose $\mathbf{y}=[\mathbf{t}, \mathbf{r}]$ and its estimate $\mathbf{\hat{y}}=[\mathbf{\hat{t}}, \mathbf{\hat{r}}]$:
\begin{equation}
\label{eq:loss_func}
	\mathcal{L} = \frac{1}{K} \sum_{k=1}^{K} ||(\mathbf{\hat{t}}_k-\mathbf{t}_k)||^2_2 + \gamma  ||(\mathbf{\hat{r}}_k-\mathbf{r}_k)||^2_2
\end{equation}
\noindent where $\norm{\cdot}$ denotes $2$-norm and $\gamma$ is a hyper-parameter to balance the weights of translation and rotation errors. Implementation details on training \monet are provided in \sect{\ref{sec:implementation}}.









